Financial Event Extraction Using Wikipedia-Based Weak Supervision

Extraction of financial and economic events from text has previously been done mostly using rule-based methods, with more recent works employing machine learning techniques. This work is in line with this latter approach, leveraging relevant Wikipedia sections to extract weak labels for sentences describing economic events. Whereas previous weakly supervised approaches required a knowledge-base of such events, or corresponding financial figures, our approach requires no such additional data, and can be employed to extract economic events related to companies which are not even mentioned in the training data.

==> results.tex <==
\section{Results}\label{sec:results}

\subsection{End-to-end system}
We evaluate the end-to-end performance of the different models using two benchmarks, VLD and Wiki on the $100$ test motions.
\subsubsection{VLD}
Figure \ref{fig:VLD_test} presents the average precision of different evidence detection models as a function of the number of top candidates per motion. Precision is high for all models, with over $90\%$ precision for the top $20$ candidates. This compares to an estimated positive prior of $0.3$ among the sentences retrieved from the queries\footnote{The estimate is based on labelling $10$ random sentences for each of the $100$ test motions}. The best performing model is \BertSM, with precision values that clearly surpass those obtained by the \BAMaskS model used by \citet{shnarch-etal-2018-will}. Notice that the \BAMaskS model receives only the masked sentence as input, while \BertSM receives the unmasked sentence and the motion. 
As expected, both BA and BERT benefit from the addition of the motion text to the input (see Figure \ref{fig:VLD_test}). 


Among the BA based models, the best results are achieved when the input is the masked sentence and the motion text (\BAMaskSM). As mentioned in Section \ref{experiment}, the advantage of masking can be attributed to the extra information it provides to the network. First, it tells the network where the topic is located within the sentence. Second, the topic may appear in multiple textual forms. For example, the topic “capital punishment” may appear in the text as “execution”, “death penalty” etc. Replacing Wikified instances of the topic with a single mask saves the need to learn the equivalence between the different forms. Finally, the usage of the same masking token for all topics can help the network learn general, motion-independent features of evidence texts.

In the case of BERT, the masking hinders the network performance. Models that are fed with masked sentences are inferior to \BertSM, which receives an unmasked sentence and a motion. A possible explanation for the negative effect of masking on BERT is that its strong underlying language model enables it to deduce the aforementioned information provided by masking from the original unmasked string. Consequently, the information that is lost in the masking process, i.e. the masked tokens, leads to inferior results.

%\input{precision_table}

It is also interesting to evaluate to what extent the direct sentence-retrieval approach differs from one based on document-retrieval. In other words, do high-ranking sentences come from a wide range of documents and journals, or is this approach {\em de-facto} similar to the document-based one, with high-ranking sentences originating in only a small number of documents? 
Our results clearly indicate that the former is true. For example, the top $20$ and top $40$ ranked candidates per motion from the \BAMaskS model originate from an average of 18.03 and 36.07 different documents, respectively.
(see supplementary for further details.)

%\begin{figure}[ht!]
%\centering
%\includegraphics[width=75mm]{average_number_art_%sources.png}
%\caption{Average number of documents and journals from which the top $k$ candidates originate, as a function of $k$. 
%\label{fig:diversity}}
%\end{figure}

\begin{figure}[ht!]
\centering
\hspace*{-3mm}\includegraphics[width=86mm]{graphs/VLD_test_with_no_duplicates.png}
\caption{VLD: Precision of top $k$ candidates vs. $k$ for different evidence
detection models. %The dataset used for training is denoted in parentheses.
\label{fig:VLD_test}}
\end{figure}


\begin{figure}[ht!]
\centering
\hspace*{-3mm}\includegraphics[width=86mm]{graphs/wiki_test_with_no_duplicates.png}
\caption{Wiki: Precision of top $k$ candidates vs. $k$ for different evidence
detection models. The dataset used for training is denoted in parentheses. 
\label{fig:Wiki_test}}
\end{figure}

\subsubsection{Wiki}
Following the high performance of the end-to-end system on VLD, it is interesting to examine how the results are affected by moving to the smaller and more homogeneous corpus of Wiki. For this purpose we tested the models trained using VLD, on Wiki test-set. In addition we trained new models on Wiki training set and tested them on test-test.
Figure \ref{fig:Wiki_test} shows the average precision of our models vs. the number of top candidates. 
Although the precision values of the leading model are still high, they are significantly lower than those obtained in VLD. 
One reason for this precision gap is that this benchmark may be "harder", containing a smaller fraction of positive examples. Another possible reason is the difference between the distribution of sentences retrieved from VLD and Wiki. In addition, the dramatically smaller number of sentences in Wiki is likely to result in lower scores among the top ranked candidates. The lower the score the less 
likely it is that a sentence is
evidence. Indeed, the Wiki scores over the top k predictions are significantly lower than the VLD scores (t-test p-value=$3.19e^{-9}$ for $k=20$). Despite the performance differences when moving from VLD to Wiki, the hierarchy between the different models is the same. Moreover, although the test sentences are from Wiki, the models which are trained on Wiki are inferior to those trained on VLD. This can be attributed to the much larger training data of VLD (154K compared to 22K in Wiki), which compensates for the potential difference between the train and test distributions. 
\subsection{blendNet benchmark}
The \BAMaskS network used here has the same architecture as that in \cite{shnarch-etal-2018-will}. It is therefore interesting to evaluate how the differences between their work and ours - greatly expanding the training data, considering the motion explicitly and using the BERT architecture - are reflected over the benchmark based on their data. 

Table \ref{tab:acc} describes the impact of these differences. Training BA$_{MaskS}$ on the VLD improves accuracy from 74\% to 78\%. 
In other words, even though blendNet was trained on Wikipedia sentences, and the benchmark is also composed of Wikipedia sentences, the larger size of the VLD more than compensates for the change in domain.
Shifting to the BERT architecture improves accuracy to 80\%, even without adding the motion as part of the input. Finally, the best accuracy is attained when combining all three modification, for a total of 10\% increase over the original accuracy.

\input{accuracy_table}


\subsection{UKP-TUDA benchmark}
The {\em UKP-TUDA} benchmark is an interesting case study for our networks, since it is labeled for whether or not a sentence is argumentative (defined as having a clear stance w.r.t. the topic), rather than whether or not it is evidence. In particular, argumentative texts which are not {\em Study Evidence} or {\em Expert Evidence} are labeled as positive examples, but are expected to receive a low score by \BertSM. In other words, when naively used as a classifier, \BertSM is expected to accept argumentative sentences which are evidence of the appropriate type, but reject argumentative sentences which are not.

Indeed, with a threshold of $0.5$, the network obtains a precision score 
of $0.88$ and a recall score of $0.16$. To verify that the predicted positives indeed tend to be {\em evidence} and that the low recall is due to other types of argumentative sentences being rejected, we manually annotated $20$ {\em argumentative} sentences with a score above the threshold, and $20$ with a score below it (chosen uniformly at random). As expected, in the first set, 14 of the sentences are {\em Study Evidence} or {\em Expert Evidence}, while in the second set only 2 are so.

Importantly, \BertSM was trained on sentences which correspond to 
the retrieval queries, and are therefore quite different from the  sentences in the {\em UKP-TUDA} benchmark; In particular, it is not clear what fraction of the negative training examples are non-argumentative sentences. Hence, it is a bit of a mystery how such sentences will be scored. To evaluate this, we considered all sentences with a classification score below the threshold. Among those which are argumentative, the average score is $7.3\cdot10^{-2}$, while among those which are not argumentative it is $1.5\cdot10^{-2}$ (t-test p-value $< 10^{-76}$), suggesting that argumentative sentences tend to be assigned a higher score.

A different way to examine this phenomenon is by considering the precision-recall curve over this benchmark. Figure \ref{fig:stab} shows that even though the network was trained to discern {\em evidence} sentences, it also learned to prefer argumentative sentences over non-argumentative ones. The curve-points toward its right end correspond to precision-recall trade-offs similar to those reported in \citet{stab2018cross} for classifiers trained directly for this task. For example, a threshold score of $0.002$ corresponds to precision of $0.66$ and recall of $0.75$ (F1-score=$0.7$) on this curve. The preferred network in \citet{stab2018cross} achieves an average precision of $0.65$, $0.67$ average recall and $0.67$ average F1-score.

Taken together these results suggest that even though \BertSM was trained on rather different data, its ranking of the {\em UKP-TUDA} tends to be {\em Study Evidence} or {\em Expert Evidence} first, then argumentative sentences not of these types and last but not least - the non argumentative sentences. 

\begin{figure}[ht!]
\centering
\includegraphics[width=75mm]{stab-bert.png}
\caption{Precision-Recall curve of \BertSM over the {\em UKP-TUDA} benchmark. \label{fig:stab}}
\end{figure}
